On Deriving Nested Calculi for Intuitionistic Logics from Semantic Systems

This paper shows how to derive nested calculi from labelled calculi for propositional intuitionistic logic and first-order intuitionistic logic with constant domains, thus connecting the general results for labelled calculi with the more refined formalism of nested sequents. The extraction of nested calculi from labelled calculi obtains via considerations pertaining to the elimination of structural rules in labelled derivations. Each aspect of the extraction process is motivated and detailed, showing that each nested calculus inherits favorable proof-theoretic properties from its associated labelled calculus.

==> body-1.tex <==


The language $\mathcal{L}$ for propositional intuitionistic logic ($\int$) is defined via the following BNF grammar: $A ::= p \ | \ \bot \ | \ (A \lor A) \ | \ (A \land A) \ | \ (A \imp A)$, where $p$ is among a denumerable set of \emph{propositional variables} $\{p, q, r, \ldots\}$. The language admits a Kripke-style semantics~\cite{Kri65} with satisfaction and validity defined relative to relational frames and models. The details are given below:


%Pg. 140 Domain D_{\Gamma} of theory defined
%Kripke models for FO Intermediate Logics Pg. 205 of Gabbay
%~\cite{Cor89-1,Iem05,TroDal88}
\begin{definition}[Intuitionistic Frame, Model~\cite{GabSheSkv09}]\label{def:frame-model} An \emph{intuitionistic frame} is an ordered pair $F = (W,\leq)$ such that:
\begin{itemize}

\item[(i)] $W$ is a non-empty set of worlds called the \emph{domain};

\item[(ii)] $\leq$ is a reflexive and transitive binary relation on $W$;\footnote{The two properties of $\leq$ are defined as follows: (\emph{Reflexivity}) For all $w \in W$, $w \leq w$, and (\emph{Transitivity}) For all $w,u,v \in W$, if $w \leq u$ and $u \leq v$, then $w \leq v$.}
\end{itemize}

A \emph{intuitionistic model} $M$ is a tuple $(F,V)$ where $F$ is an intuitionistic frame and $V$ is a \emph{valuation function} that maps each propositional variable $p$ to a subset of $W$ such that the following \emph{monotonicity condition} holds: If $w \leq v$ and $w \in V(p)$, then $v \in V(p)$.
%\begin{flushleft}
%$\mathbf{(M)}$ \ \ If $w \leq v$ and $w \in V(p)$, then $v \in V(p)$.
%Def 3.2.8, p. 207 Gabbay for (TP) above
%\end{flushleft}
\end{definition}




%Semantic Clauses found on pp. 208-209 of Gabbay
%~\cite{Cor89-1,Iem05,Kri65,TroDal88}
\begin{definition}[Semantic Clauses~\cite{GabSheSkv09}]\label{def:semantic-clauses} Let $M$ be an intuitionistic model with $w \in W$ of $M$. We inductively define the \emph{satisfaction} of a formula as follows:

\begin{itemize}

\item[(i)] $M,w \not\Vdash \bot$

\item[(ii)] If $p$ is a propositional variable, then $M,w \Vdash p$ iff $w \in V(p)$;

\item[(iii)] $M,w \Vdash A \vee B$ iff $M,w \Vdash A$ or $M,w \Vdash B$;

\item[(iv)] $M,w \Vdash A \land B$ iff $M,w \Vdash A$ and $M,w \Vdash B$;

\item[(v)] $M,w \Vdash A \imp B$ iff for all $u \in W$, if $w \leq u$ and $M,u \Vdash A$, then $M,u \Vdash B$;

\end{itemize}


We say that a formula $A$ is \emph{globally true on $M$}, written $M \Vdash A$, iff $M,u \Vdash A$ for all worlds $u \in W$. A formula $A$ is \emph{valid}, written $ \Vdash A$, iff it is globally true on all intuitionistic models.

We say that a set $\Theta$ of formulae \emph{semantically implies} a formula $A$, written $\Theta \Vdash A$, iff for all intuitionistic models $M$ with $w \in W$ of $M$, if $M,w \Vdash B$ for all $B \in \Theta$, then $M,w \Vdash A$.

\end{definition}

By Def.~\ref{def:semantic-clauses} above, the monotonicity condition of Def.~\ref{def:frame-model} can be restated as: for any intuitionistic model $M$ with $w$ and $v$ in the domain $W$ of $M$, if $w \leq v$ and $M,w \Vdash p$, then $M,v \Vdash p$. It is a useful fact that this statement generalizes to arbitrary formulae, and will be leveraged in Section~\ref{section-3} when deriving the nested calculus from the labelled calculus.

%Lem 3.2.16 Gabbay (p. 209)
\begin{lemma}[General Monotonicity~\cite{GabSheSkv09}]\label{lm:persistency} %~{\cite[Lem.~3.2.16]{GabSheSkv09}}]
\label{lm:persistency} Let $M$ be a model with domain $W$ and $w,u \in W$. If $w \leq u$ and $M,w \Vdash A$, then $M,u \Vdash A$.

\end{lemma}

Furthermore, propositional intuitionistic logic admits a finite axiomatization. The axioms and inference rule characterizing $\int$ are given in Fig.~\ref{fig:intuitionistic-axioms}.

\begin{figure}
\noindent\hrule
$$
A \supset (B \supset A)
\qquad
(A \imp (B \imp C)) \imp ((A \imp B) \imp (A \imp C))
\qquad
A \supset (B \supset (A \land B))
$$
$$
(A \land B) \supset A
\qquad
(A \land B) \supset B
\qquad
A \supset (A \lor B)
\qquad
B \supset (A \lor B)
\qquad
\bot \imp A
$$
$$
(A \supset C) \supset ((B \supset C) \supset ((A \lor B) \supset C))
\qquad
\AxiomC{$A$}
\AxiomC{$A \imp B$}
\RightLabel{$(mp)$}
\BinaryInfC{$B$}
\DisplayProof
$$

\hrule
\caption{The axiomatization of propositional intuitionistic logic $\int$.}\label{fig:intuitionistic-axioms}
\end{figure}



We define a \emph{derivation in $\int$} from a set of premises $\Theta$ (written $\Theta \vdash A$) to be a sequence of formulae $B_{0}, \ldots, B_{n}$ such that (i) $B_{i}$ is an instance of an axiom, (ii) $B_{i}$ is an element of $\Theta$, or (iii) $B_{i}$ is obtained from an application of $(mp)$ on formulae $B_{j}$ and $B_{k}$ with $j,k < i$, for $i \in \{0, \ldots, n\}$. We say that a formula $A$ is a \emph{theorem} of $\int$, and write $\vdash A$, if and only if there exists a derivation of $A$ in $\int$ from the empty set $\emptyset$ of premises.

%All three logics are equivalently characterizable by means of a Kripke-style semantics. However, to avoid overburdening this paper with extensive background details, the semantics, soundness, and completeness of $\int$, $\intfo$, and $\intfocd$ are provided in App.~\ref{app:semantics} for the interested reader.

%Soundness discussed around pg. 214 of Gabbay
%Lem. 3.2.31 Gabbay (p. 218)
\begin{theorem}[Soundness and Completeness~\cite{GabSheSkv09}] For any $A \in \mathcal{L}$, $\Theta \Vdash A$ iff $\Theta \vdash A$.

\end{theorem}
